LLN: Learnable Lens Networks for Parameter-Efficient Long-Horizon Dynamical Prediction

Explicit residual connections of the form (x+f(x)), often combined with normalization layers, have become a standard strategy for training very deep neural networks. However, residual addition primarily provides an algebraic shortcut for gradient propagation, while leaving the evolution of feature geometry across layers largely unconstrained. We introduce Learnable Lens Networks (LLN), a physics-inspired architecture that replaces direct feature-space residual accumulation with learnable optical transport in an augmented position-angle phase space. Each layer alternates between free propagation, which provides an implicit transport path, and a learnable lens field that performs nonlinear trajectory transformation and focusing. Theoretically, we establish that LLN transport is globally invertible and volume-preserving for any differentiable lens field, with the implemented coordinate-wise Gaussian transport further satisfying symplecticity. Importantly, these structural constraints do not limit expressivity: with unrestricted embeddings and readouts, LLN retain universal approximation of continuous end-to-end maps. Experiments across diverse dynamical systems demonstrate that LLN improves long-horizon prediction while using substantially fewer parameters than same-depth comparators. Further analysis reveals stable depth-wise gradient transport and interpretable learned dynamics under the coupled propagation and refraction design.

==> tables/kan_transition_baseline_table.tex <==
\begin{center}
\begin{minipage}{\textwidth}
\centering
\footnotesize
\captionof{table}{\textbf{Contemporary functional transition baseline on the ten-system benchmark.} The RBF/KAN-style delta predictor uses the same state-to-state training pairs, depth $D=40$, seed set, and 500-step normalized rollout metric as the main dynamics protocol. Its low one-step errors show that local transition fitting alone does not ensure stable closed-loop rollouts. Lower rollout MSE is better; bold marks the lower closed-loop rollout MSE and LLN-favorable ratios.}
\label{tab:kan_transition_baseline}
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
System & KAN one-step & RBF/KAN rollout & LLN rollout & LLN/KAN & KAN params \\
\midrule
Lorenz-24 & $0.015$ & $14.441\!\pm\!5.086$ & \textbf{$6.170\!\pm\!0.953$} & \textbf{$0.427$} & 1,319,019 \\
Lorenz-28 & $1.98{\times}10^{-3}$ & $98.970\!\pm\!131.090$ & \textbf{$0.920\!\pm\!0.545$} & \textbf{$9.30{\times}10^{-3}$} & 1,319,019 \\
SpringChain-32 & $8.32{\times}10^{-5}$ & $12.112\!\pm\!4.281$ & \textbf{$1.070\!\pm\!0.379$} & \textbf{$0.088$} & 1,326,888 \\
SpringChain-48 & $6.38{\times}10^{-5}$ & $9.772\!\pm\!4.108$ & \textbf{$1.087\!\pm\!0.017$} & \textbf{$0.111$} & 1,331,016 \\
Burgers-32 & $1.01{\times}10^{-4}$ & $21.387\!\pm\!6.513$ & \textbf{$0.537\!\pm\!0.155$} & \textbf{$0.025$} & 1,322,760 \\
Burgers-48 & $7.28{\times}10^{-5}$ & $15.238\!\pm\!4.438$ & \textbf{$0.550\!\pm\!0.122$} & \textbf{$0.036$} & 1,324,824 \\
AdvecDiff-32 & $8.23{\times}10^{-5}$ & $22.847\!\pm\!9.039$ & \textbf{$0.962\!\pm\!0.596$} & \textbf{$0.042$} & 1,322,760 \\
AdvecDiff-48 & $7.64{\times}10^{-5}$ & $16.555\!\pm\!6.902$ & \textbf{$0.564\!\pm\!0.318$} & \textbf{$0.034$} & 1,324,824 \\
ReactionDiff-32 & $8.57{\times}10^{-5}$ & $26.453\!\pm\!11.712$ & \textbf{$0.065\!\pm\!0.042$} & \textbf{$2.46{\times}10^{-3}$} & 1,322,760 \\
ReactionDiff-48 & $7.55{\times}10^{-5}$ & $17.710\!\pm\!4.736$ & \textbf{$0.042\!\pm\!0.031$} & \textbf{$2.37{\times}10^{-3}$} & 1,324,824 \\
\bottomrule
\end{tabular}
}
\vspace{0.25em}
\parbox{0.98\textwidth}{\raggedright\footnotesize
\emph{Configuration.} RBF/KAN uses hidden width 64, 8 Gaussian basis functions per hidden coordinate, Adam training for 6 epochs, bounded delta magnitude 0.1, and delta-form prediction in standardized coordinates; all rows have 10/10 finite seeds.}
\end{minipage}
\end{center}

